Who's Who: Large Language Models Meet Knowledge Conflicts in Practice

Retrieval-augmented generation (RAG) methods are viable solutions for addressing the static memory limits of pre-trained language models. Nevertheless, encountering conflicting sources of information within the retrieval context is an inevitable practical challenge. In such situations, the language models are recommended to transparently inform users about the conflicts rather than autonomously deciding what to present based on their inherent biases. To analyze how current large language models (LLMs) align with our recommendation, we introduce WhoQA, a public benchmark dataset to examine model's behavior in knowledge conflict situations. We induce conflicts by asking about a common property among entities having the same name, resulting in questions with up to 8 distinctive answers. WhoQA evaluation set includes 5K questions across 13 Wikidata property types and 150K Wikipedia entities. Our experiments show that despite the simplicity of WhoQA questions, knowledge conflicts significantly degrades LLMs' performance in RAG settings.

==> Sections/4_ConstructionProcess.tex <==
\paragraph{Question-Answer pairs collection:} In Wikidata, each relation is represented by an $(s, r, E)$ triplet. We choose relations whose the set $E$ contains Wikidata entities, plain texts or a date time string. For each relation, we create 5 question templates. See details of these question templates in Appendix \ref{appendix:qtemplates}. And for each entity set E, we include all Wikipedia-recommended answer variations for our evaluation robustness. This step generates approximately 293,000 question quadruplets $(q, E, S, D)$, highlighting the prevalence of knowledge conflicts in practice.

\paragraph{Supporting evidence collection:} For each Wikipedia document $d_i$ in a question quadruplet, we search for all occurrences of the corresponding set $E_j$ and
take paragraphs of 256 tokens around the most frequent answer as candidate supporting evidence. Then, we concatenate the question with the expected answer and use Contriever \cite{izacard2021contriever} to calculate candidate paragraphs' relevant score. We keep only the most relevant paragraph in $d_i$, if its score is above 0.45. Otherwise, $d_i$ and $E_j$ are removed from our dataset. Finally, we filter the set $E_j$ to include answers appearing together with the most frequent answer in the top-1 paragraph. Our straightforward matching process, typically results in supporting documents where the answers can be found directly stated.

\paragraph{Final Benchmark:}
After all the filtering steps, WhoQA consists of 76,487 questions belonging to 13 different relations and involving 145,710 different Wikidata entities. To study the effect of relation types and the number the of conflicting answers to LLMs performance, we under sample relations with many questions and prioritize questions with many conflicting answers. For each relation, we randomly take at most 500 questions and perform weighted sampling, where questions with a higher number of conflicting answers are assigned a greater probability of being selected.

To ensure reliability of the evaluation set, we hire 2 annotators to independently check if the automatically collected supporting evidence really supports the answers from Wikidata. Originally we have 18,967 documents to check. To save time, we simply drop a whole question together with all its documents, if there is at least one incorrectly labeled document. In total, we found 479 incorrectly labeled documents, and agreed on excluding of 1602 documents. Our post checking process finally returns an evaluation set containing 5152 questions, with 3.25 conflicting answers per question on average. See the detail of our dataset statistics in Appendix \ref{}

